Phantom Embeddings: Using Embedding Space for Model Regularization in Deep Neural Networks

The strength of machine learning models stems from their ability to learn complex function approximations from data; however, this strength also makes training deep neural networks challenging. Notably, the complex models tend to memorize the training data, which results in poor regularization performance on test data. The regularization techniques such as L1, L2, dropout, etc. are proposed to reduce the overfitting effect; however, they bring in additional hyperparameters tuning complexity. These methods also fall short when the inter-class similarity is high due to the underlying data distribution, leading to a less accurate model. In this paper, we present a novel approach to regularize the models by leveraging the information-rich latent embeddings and their high intra-class correlation. We create phantom embeddings from a subset of homogenous samples and use these phantom embeddings to decrease the inter-class similarity of instances in their latent embedding space. The resulting models generalize better as a combination of their embedding and regularize them without requiring an expensive hyperparameter search. We evaluate our method on two popular and challenging image classification datasets (CIFAR and FashionMNIST) and show how our approach outperforms the standard baselines while displaying better training behavior.

==> scratchPad <==
\begin{figure}
\centering
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/dellen1.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/kratzer1.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/steinschlag1.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/abrieb1.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/brandloch2.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/marderschaden2.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/verformt1.jpg} \\
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/verschmutzt1.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/verschlissen2.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/verkratzt1.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/delle1.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/korrosion1.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/gebrochen1.jpg}
        \includegraphics[height=1.5cm, width=1.5cm]{figs/crops/lackmangel2.jpg}
\caption{Crops of damages}
\label{fig:bbox}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\caption{Table captions should be placed above the
tables.}\label{tab1}
\begin{tabular}{|l|l|l|}
\hline
Heading level &  Example & Font size and style\\
\hline
Title (centered) &  {\Large\bfseries Lecture Notes} & 14 point, bold\\
1st-level heading &  {\large\bfseries 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bfseries 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bfseries Run-in Heading in Bold.} Text follows & 10 point, bold\\
4th-level heading & {\itshape Lowest Level Heading.} Text follows & 10 point, italic\\
\hline
\end{tabular}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

